Accelerating Graph Sampling for Graph Machine Learning using GPUs

Representation learning algorithms automatically learn the features of data. Several representation learning algorithms for graph data, such as DeepWalk, node2vec, and GraphSAGE, sample the graph to produce mini-batches that are suitable for training a DNN. However, sampling time can be a significant fraction of training time, and existing systems do not efficiently parallelize sampling. Sampling is an embarrassingly parallel problem and may appear to lend itself to GPU acceleration, but the irregularity of graphs makes it hard to use GPU resources effectively. This paper presents NextDoor, a system designed to effectively perform graph sampling on GPUs. NextDoor employs a new approach to graph sampling that we call transit-parallelism, which allows load balancing and caching of edges. NextDoor provides end-users with a high-level abstraction for writing a variety of graph sampling algorithms. We implement several graph sampling applications, and show that NextDoor runs them orders of magnitude faster than existing systems.

==> algos/k-hop-GS.tex <==
% !TEX root = ../main.tex

\begin{figure}[t]
  \small
      \begin{lstlisting}[language=NextDoorAPI]
int steps() {return 2;} |\label{line:sage:steps}|
int sampleSize(k) {return (k == 0) ? 25 : 10;}|\label{line:sage:maxsize}|
Vertex next(k, src, root, srcEdges, neighbrId,
            sampler) |\label{line:sage:begin}|
{
  int idx;
  idx = randInt(0, srcEdges.size() - 1);
  return srcEdges[idx];
}|\label{line:sage:end}|

bool distinct(root) {return false;} |\label{line:sage:distinct}|
int previousSteps(int prevSteps) {return 0;}
      \end{lstlisting}
  \caption{GrapSAGE's 2-hop neighbors in \sysname{}}
  \label{fig:2-hop-sage}
\end{figure}


==> algos/k-hop.tex <==
% !TEX root = ../main.tex

\begin{figure}[t]
  \small
      \begin{lstlisting}[language=NextDoorAPI]
int steps() {return 2;} |\label{line:2-hops-steps}|
int sampleSize(k) {return ALL;}|\label{line:2-hops-maxsize}|
Vertex next(k, src, root, srcEdges, neighbrId,
            sampler) |\label{line:2-hops-next-begin}|
{ return srcEdges[neighbrId]; }|\label{line:2-hops-next-end}|

bool distinct(root) {return true;} |\label{line:2-hops-remove-duplicates}|

      \end{lstlisting}
  \caption{Finding all 2-hop neighbors in a graph in \sysname{} }
  \label{fig:2-hop-neighbors}
\end{figure}


==> algos/source-parallel-new.tex <==
% !TEX root = ../main.tex

\begin{algorithm}[t]
\caption{\Source-Parallel Sampling}
\label{algo:source-parallel}
\begin{algorithmic}[1]
\State{$G(V,E)$: the input graph; $G.E[v]$:  neighbors of $v \in V$}
\State{$S$: the samples, $S \subseteq 2^G$}
\State{$k$: the number of steps}
\State{$N$: $N[i]$ is the number of neighbors to sample at step $i$}
\State{$\fnext(s,t,G.E[t])$: the user-defined function}
\Function{TransitParallel}{$G,S,k,N$, $\fnext$}
  \State{$T \gets \langle s \mapsto \{v \mid s\in S, v\in S\} \rangle$}
  \Comment{sample to transits map}
  \State{$M \gets invert(T)$}
  \Comment{transit to samples map}
  \For{$i \in 0\cdots k$}
    \ParFor{$s \in \textsc{Keys}(T)$}
      \State{$T[s] \gets \emptyset$}
    \EndParFor
    \ParFor{$t \in \textsc{Keys}(M)$} \Comment{each $t$ in a block}
      \ParFor{$s \in M[t]$} \Comment{each $s$ in a (sub-)warp}
        \State{$\mathit{newTransits} \gets \emptyset$}
        \ParFor{$j \in 1\cdots N[i]$} \Comment{each in thread}
          \State{$u\gets \fnext(s,t,G.E[t])$}
          \State{$\mathit{newTransits} \gets\mathit{newTransits} \cup \{u\}$}
        \EndParFor
      \State{$s \gets s \cup \mathit{newTransits}$}
      \State{$T[s] \gets T[s] \cup \mathit{newTransits}$}
      \EndParFor
    \EndParFor
    \State{$M \gets invert(T)$} \label{ln:invert}
  \EndFor
  \State{\textbf{return}~$S$}
\EndFunction
  % \State{\texttt{/* thread block $b$ */}}
  % \ParFor{\source vertex $v$}
  %   \State{\texttt{/* thread $t$ of $b$ */}}
  %   \ParFor{sample $s$ having $v$ as transit}
  %     \If{$N(v)$ not cached in shared memory}
  %       \State{move $N(v)$ from global to shared memory}
  %     \EndIf
  %     \State{\texttt{/* $N(v)$ accessed from shared memory */}}
  %     \State{$D$ $\gets$ \texttt{next}($s$, $v$, $N(v)$)}
  %     \State{add $D$ to $s$ in global memory}
  %   \EndParFor
  % \EndParFor
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}[t]
%   \caption{Source-Centric Computation Step $i$}
%   \label{algo:source-centric}
%   \begin{algorithmic}[1]
%     \State{$I_v$ $\gets$ set of source vertices in samples of size $i-1$}
%     \ParFor{$v \in I_v$}
%       \ForAll{sample $s$ to be expanded using $v$}
%         \State{$s$ $\gets$ $s$ $\cup$ one or more neighbors of $v$}
%       \EndFor
%       \State{output $s$}
%     \EndParFor
%   \end{algorithmic}
% \end{algorithm}


==> algos/system-algo.tex <==
% !TEX root = ../main.tex

\begin{algorithm}[h]
  \caption{\sysname{}'s Algorithm}
  \label{algo:nextdoor}
  \textbf{Input}: $G (V, E)$ input graph\\
  \textbf{Input}: Implementation of \texttt{steps}, \texttt{maxSize}, \texttt{next}, and \texttt{distinct}\\
  \textbf{Output}: Sample set for each vertex
  \begin{algorithmic}[1]
    \State{SampleSet $\gets \phi$} \label{line:algo:nextdoor:sample-set-init}
    \ForAll {k = 0 $\to$ \texttt{steps}()} \label{line:algo:nextdoor:all-steps-begin}
      % \ForAll {v $\in$ G} \label{line:algo:nextdoor:sample-set-init-begin}
      %   \State{SampleSet$_v^{k} \gets \phi$}
      % \EndFor \label{line:algo:nextdoor:sample-set-init-end}
      \State{SampleSet$^{k}$ $\gets$ \textsc{AllocSampleSet$_{CPU}$}(G$^{R}_i$, \texttt{maxSize})} \label{line:algo:nextdoor:sample-set-offsets}
      \State{$\mathcal{G}_N$ $\gets$ \textsc{PartitionGraph$_{CPU}$}(G, SampleSet$^{k}$)} \label{line:algo:nextdoor:partition}
      \ForAll {G$^{R}_{i}$ $\in$ $\mathcal{G}_N$}\label{line:algo:nextdoor:all-parts-begin}
        \State{srcToRoots $\gets$ \textsc{SrcToRoots$_{CPU}$}($\cup_{v \in G^{R}_i}$ SampleSet$_v^{k-1}$)} \label{line:algo:nextdoor:src-to-roots}
        \State{[G$_{1}^{S}$ \ldots G$_{N}^{S}$] $\gets$ \textsc{SrcGraphs$_{CPU}$}(srcToRoots)} \label{line:algo:nextdoor:src-graphs}
        \State{nextSampleSet $\gets \phi$}
        \ForAll{G$_{j}^{S} \in$ [G$_{1}^{S} \ldots$ G$_{N}^{S}$]} \label{line:algo:nextdoor:for-all-src-graphs}
          \State{nextSampleSet $\gets$ nextSampleSet $\cup$ \textsc{NextNeighbors$_{GPU}$}(G$_{j}^{S}$, srcToRoots, \texttt{next})} \label{line:algo:nextdoor:next}
        \EndFor
        \State{SampleSet$^{k}$ $\gets$ \textsc{Unique$_{GPU}$}(nextSampleSet, \texttt{distinct})} \label{line:algo:nextdoor:remove-duplicates}
      \EndFor\label{line:algo:nextdoor:all-parts-end}
    \EndFor \label{line:algo:nextdoor:all-steps-end}
    \State{\Return{SampleSet}}
  \end{algorithmic}
\end{algorithm}

